On Practical Nearest Sub-Trajectory Queries under the Fr\'echet Distance

We study the problem of sub-trajectory nearest-neighbor queries on polygonal curves under the continuous Fr\'echet distance. Given an $n$ vertex trajectory $P$ and an $m$ vertex query trajectory $Q$, we seek to report a vertex-aligned sub-trajectory $P'$ of $P$ that is closest to $Q$, i.e. $P'$ must start and end on contiguous vertices of $P$. Since in real data $P$ typically contains a very large number of vertices, we focus on answering queries, without restrictions on $P$ or $Q$, using only precomputed structures of ${\mathcal{O}}(n)$ size. We use three baseline algorithms from straightforward extensions of known work, however they have impractical performance on realistic inputs. Therefore, we propose a new Hierarchical Simplification Tree data structure and an adaptive clustering based query algorithm that efficiently explores relevant parts of $P$. The core of our query methods is a novel greedy-backtracking algorithm that solves the Fr\'echet decision problem using ${\cal O}(n+m)$ space and ${\cal O}(nm)$ time in the worst case. Experiments on real and synthetic data show that our heuristic effectively prunes the search space and greatly reduces computations compared to baseline approaches.

==> Figs/canon_eg.tex <==
\begin{figure}\centering
    \includegraphics[scale=0.6]{./Figs/canon_eg.pdf} \\
	\caption{Freespace diagram example showing a trajectory $P$ ($|P|=22$) and query $Q$ ($|Q|=18$) from the Pen Tip~\cite{pentip06} data set. 
	In this example, point $(q_m,p_n)$ is reachable from point $(q_1,p_1)$ via the canonical path (green).
	}
	\todo[inline]{Inconsistent. Make canonical path blue. The Pen~Tip data set is not used in this study. Use Pigeon or Football ?}
	\label{fig:canon_eg}
% 	\vspace{-1em}
\end{figure}


==> Figs/fig_query_results.tex <==

\begin{figure}[h]
% \vspace{-0.05cm}
%%%%%%%%%%%%%%%%%%%
% Main sub-trajectory Query Results
%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}

\begin{groupplot}[
     group style = {group size = 4 by 3,
                    horizontal sep=0.15cm,
                    vertical sep=0.15cm,},
     height=4.0cm,
     width=3.2cm,
     grid style=dashed,
    %  sharp plot,
     stack plots = false,
     xmode = normal,
     xtick=data,
     xtick style={draw=none},
     xticklabels={,,},
     xmin=0.5, xmax=3.5,
     ymode = log,
     ymin=20, ymax=1500,
     ytick={10,100,1000},
     ymajorgrids=true,
     log ticks with fixed point,
     log origin = infty,
    ]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Runtime per query (ms)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   

%%%%%%%%%%%%%%%%%%%
% Pigeon
%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,$10^{1}$,$10^{2}$,$10^{3}$,$10^{4}$,$10^{5}$},
ymin=5, ymax=50000,
ytick={1,10,100,1000,10000,100000},
ylabel={Runtime (ms)},
]

\addplot[color=black,mark=star,]
coordinates {(1,718)(2,9350)};

\addplot[color=black,mark=diamond,]
coordinates {(1,486)(2,7291)};

\addplot[color=black,mark=otimes,]
coordinates {(1,798)};

\addplot[color=blue,mark=o,]
coordinates {(1,70)(2,441)(3,3825)};

\addplot[color=blue,mark=square,]
coordinates {(1,164)(2,253)(3,488)};

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Football
%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,,},
ymin=5, ymax=50000,
ytick={1,10,100,1000,10000,100000},
legend style={at={(0.95,1.44)},anchor=north},
legend columns = 3,
]

\addplot[color=black,mark=star,]
coordinates {(1,891)(2,12342)};

\addplot[color=black,mark=diamond,]
coordinates {(1,439)(2,6554)};

\addplot[color=black,mark=otimes,]
coordinates {(1,15)};

\addplot[color=blue,mark=o,]
coordinates {(1,67)(2,564)(3,5468)};

\addplot[color=blue,mark=triangle,]
coordinates {(1,2127)};

\addplot[color=blue,mark=square,]
coordinates {(1,122)(2,211)(3,546)};

\legend{Baseline $1$}
\addlegendentry{Baseline $2$}
\addlegendentry{Baseline $3$}
\addlegendentry{Algorithm $1$}
\addlegendentry{Algorithm $2$}
\addlegendentry{Algorithm $3$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthetic (low)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,,},
ymin=5, ymax=50000,
ytick={1,10,100,1000,10000,100000},
]

\addplot[color=black,mark=star,]
coordinates {(1,1011)(2,14417)};

\addplot[color=black,mark=diamond,]
coordinates {(1,596)(2,7125)};

\addplot[color=black,mark=otimes,]
coordinates {(1,8)};

\addplot[color=blue,mark=o,]
coordinates {(1,86)(2,697)(3,7550)};

\addplot[color=blue,mark=triangle,]
coordinates {(1,200)(2,628)};

\addplot[color=blue,mark=square,]
coordinates {(1,194)(2,259)(3,386)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthetic (high)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,,},
ymin=5, ymax=50000,
ytick={1,10,100,1000,10000,100000},
]

\addplot[color=black,mark=star,]
coordinates {(1,448)(2,4971)};

\addplot[color=black,mark=diamond,]
coordinates {(1,260)(2,2901)};

\addplot[color=black,mark=otimes,]
coordinates {(1,19)};

\addplot[color=blue,mark=o,]
coordinates {(1,60)(2,545)(3,4947)};

\addplot[color=blue,mark=triangle,]
coordinates {(1,5213)};

\addplot[color=blue,mark=square,]
coordinates {(1,99)(2,102)(3,956)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Number of operations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  

%%%%%%%%%%%%%%%%%%%
% Pigeon
%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,$10^{0}$,$10^{1}$,$10^{2}$,$10^{3}$,$10^{4}$},
ymin=0.5, ymax=15000,
ytick={0.1,1,10,100,1000,10000},
ylabel={Nof. Operations},
]

\addplot[color=black,mark=star,]
coordinates {(1,460.0)(2,638.3)};

\addplot[color=black,mark=diamond,]
coordinates {(1,423.3)(2,499.0)};

\addplot[color=blue,mark=o,]
coordinates {(1,36.5)(2,32.3)(3,31.6)};

\addplot[color=blue,mark=square,]
coordinates {(1,108.0)(2,7.2)(3,1.2)};

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Football
%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,,},
ymin=0.5, ymax=15000,
ytick={0.1,1,10,100,1000,10000},
]

\addplot[color=black,mark=star,]
coordinates {(1,583.9)(2,829.7)};

\addplot[color=black,mark=diamond,]
coordinates {(1,294.4)(2,426.1)};

\addplot[color=blue,mark=o,]
coordinates {(1,45.7)(2,44.4)(3,44.0)};

\addplot[color=blue,mark=triangle,]
coordinates {(1,473.6)};

\addplot[color=blue,mark=square,]
coordinates {(1,72.5)(2,5.9)(3,1.1)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthetic (low)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,,},
ymin=0.5, ymax=15000,
ytick={0.1,1,10,100,1000,10000},
]

\addplot[color=black,mark=star,]
coordinates {(1,682.8)(2,985.9)};

\addplot[color=black,mark=diamond,]
coordinates {(1,345.2)(2,488.8)};

\addplot[color=blue,mark=o,]
coordinates {(1,52.8)(2,52.4)(3,56.5)};

\addplot[color=blue,mark=triangle,]
coordinates {(1,81.1)(2,20.6)};

\addplot[color=blue,mark=square,]
coordinates {(1,147.1)(2,19.3)(3,2.8)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthetic (high)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
yticklabels={,,},
ymin=0.5, ymax=15000,
ytick={0.1,1,10,100,1000,10000},
]
	
\addplot[color=black,mark=star,]
coordinates {(1,272.1)(2,310.8)};

\addplot[color=black,mark=diamond,]
coordinates {(1,153.6)(2,177.5)};

\addplot[color=blue,mark=o,]
coordinates {(1,41.1)(2,40.2)(3,40.0)};

\addplot[color=blue,mark=triangle,]
coordinates {(1,1080.7)};

\addplot[color=blue,mark=square,]
coordinates {(1,58.9)(2,2.5)(3,5.1)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Avg Max |c| per query
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
% Pigeon
%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
xlabel={Pigeon},
xticklabels={$10^3$,$10^4$,$10^5$},
yticklabels={,$10^{2}$,$10^{3}$},
ylabel={Max $|c|$},
height=3.0cm,
]

\addplot[color=blue,mark=square,]
coordinates {(1,62)(2,88)(3,259)};

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Football
%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
xlabel={Football},
xticklabels={$10^3$,$10^4$,$10^5$},
yticklabels={,,},
height=3.0cm,
]

\addplot[color=blue,mark=square,]
coordinates {(1,49)(2,113)(3,336)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthetic (low)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
xlabel={Synth. low},
xticklabels={$10^3$,$10^4$,$10^5$},
yticklabels={,,},
height=3.0cm,
]

\addplot[color=blue,mark=square,]
coordinates {(1,34)(2,42)(3,48)};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthetic (high)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
xlabel={Synth. high},
xticklabels={$10^3$,$10^4$,$10^5$},
yticklabels={,,},
height=3.0cm,
]

\addplot[color=blue,mark=square,]
coordinates {(1,96)(2,129)(3,886)};

\end{groupplot}
\end{tikzpicture}
\vspace{-.4cm}
\caption{Nearest-neighbor sub-trajectory query results, showing averages over $1$,$000$ queries, for baseline and proposed algorithms.
{\normalfont
Rows denote query runtime in ms (top), number of query operations as a factor of $|P|$ (middle), and maximum candidate $|c|$ sizes (bottom).
Columns (from left to right) show the Pigeon and Football real data sets and Synthetic low and high intrinsic dimensionality data sets, with $|P|=$ $10^3$, $10^4$, and $10^5$ for each.
Baseline $2$ is a $2$-approximation.
Experiments are stopped and results omitted if queries take longer than 20 seconds on average.
Baseline $3$ experiments $|P|=$ $10^4$ and $10^5$ cannot be run (quadratic-size CCT issue).
}
}
\label{fig:query_results}
\end{figure}


==> Figs/fs1.tex <==
\begin{figure}\centering
	\includegraphics[width=.45\textwidth,height=16.0cm]{./Figs/fs1_curves.png} 
	\hspace{1.0cm}
    \includegraphics[width=.45\textwidth,height=16.0cm]{./Figs/fs1.pdf} \\
	\caption{Freespace diagram example showing an input trajectory $P$ (black, $|P|=30$) and query $Q$ (blue, $|Q|=8$) from the Football~\cite{soccer15} data set. 
	The left-side shows the trajectory plots, with the $CF$ distance between $P$ and $Q$, and the $\tau$ distance used to generate the freespace diagram.
	The right-side shows the freespace diagram between $P$ and $Q$ for the given $\tau$ distance, with freespace in white and non-freespace in grey (grid-lines correspond to $P$ and $Q$ vertices).
	In this example point $(q_m,p_n)$ is reachable from point $(q_1,p_1)$.
	Note that for simplicity, freespace cell plots show straight edges (technically they are ellipses).
	}
	\todo[inline]{In the journal version, this should only be in the appendix (if at all).}
	\label{fig:fs1}
% 	\vspace{-1em}
\end{figure}


==> Figs/vert_ray.tex <==


